Domain-matched Pre-training Tasks for Dense Retrieval

Pre-training on larger datasets with ever increasing model size is now a proven recipe for increased performance across almost all NLP tasks. A notable exception is information retrieval, where additional pre-training has so far failed to produce convincing results. We show that, with the right pre-training setup, this barrier can be overcome. We demonstrate this by pre-training large bi-encoder models on 1) a recently released set of 65 million synthetically generated questions, and 2) 200 million post-comment pairs from a preexisting dataset of Reddit conversations made available by pushshift.io. We evaluate on a set of information retrieval and dialogue retrieval benchmarks, showing substantial improvements over supervised baselines.

==> tables/pretraining_reddit.tex <==
\begin{table}[ht]
\centering

\begin{tabular}{llccc}
 \toprule
\multirow{2}*{\textbf{Model}}         & 
\multirow{2}*{\textbf{Task}} & \textbf{ConvAI} & \textbf{DSTC} & \textbf{Ubuntu} \\
        &   & R@1        & MRR   &   MRR \\
\midrule
BERT & - & 82.6 & & \\
Roberta & - & & & \\
BERT* & MLM & 86.9 & & \\
% BERT & BiEnc & \textbf{88.7} & & \\
\hline
BERT-base & BiEnc Reddit & 88.45 & & \\
Roberta-base & BiEnc Reddit & 88.42 & & \\
BERT-large & BiEnc Reddit & 88.23 & & \\
Roberta-large & BiEnc Reddit & \textbf{90.73} & & \\

\bottomrule
\end{tabular}
\caption{Comparison of different pre-training tasks. Pre-training data is Reddit comments.
*MLM number from \citep{humeau2019poly}.}
\label{tab:pretraining_reddit}
\end{table} 
